Towards an In-Depth Comprehension of Case Relevance for Better Legal Retrieval

Legal retrieval techniques play an important role in preserving the fairness and equality of the judicial system. As an annually well-known international competition, COLIEE aims to advance the development of state-of-the-art retrieval models for legal texts. This paper elaborates on the methodology employed by the TQM team in COLIEE2024.Specifically, we explored various lexical matching and semantic retrieval models, with a focus on enhancing the understanding of case relevance. Additionally, we endeavor to integrate various features using the learning-to-rank technique. Furthermore, fine heuristic pre-processing and post-processing methods have been proposed to mitigate irrelevant information. Consequently, our methodology achieved remarkable performance in COLIEE2024, securing first place in Task 1 and third place in Task 3. We anticipate that our proposed approach can contribute valuable insights to the advancement of legal retrieval technology.

==> author_23.tex <==
\title{Towards an In-Depth Comprehension of Case Relevance for Better Legal Retrieval}
\titlerunning{Towards an In-Depth Comprehension of Case Relevance}
\author{Haitao Li\inst{1,2}\orcidID{0009-0006-8766-8610} \and
You Chen\inst{1,2}\orcidID{0009-0008-9873-4315} \and
Zhekai Ge\inst{3}\orcidID{0009-0005-5619-8591} \and
Qingyao Ai \inst{1,2}\orcidID{0000-0002-5030-709X} \and
Yiqun Liu \inst{1,2}\orcidID{0000-0002-0140-4512} \and
Quan Zhou \inst{4,2} \orcidID{0009-0003-8097-4621} \and
Shuai Huo \inst{4,2} \orcidID{0009-0007-1276-0268}
}

\authorrunning{Li. Author et al.}

\institute{DCST, Tsinghua University, China \and
Quan Cheng Laboratory, China \and
Columbia University, USA \and
MegaTech.AI, China \\
\email{liht22@mails.tsinghua.edu.cn}
}

\index{Li, Haitao}
\index{Chen, You}
\index{Ge, Zhekai}
\index{Ai, Qingyao}
\index{Liu, Yiqun}
\index{Zhou, Quan}
\index{Huo, Shuai}
\numberofpages{16}

\contactauthor{Liu, Yiqun}
\contactemail{yiqunliu@tsinghua.edu.cn}
\contentfolder{COLIEE2024camera/}
\contentfilename{COLIEE2024camera/COLIEE2024camera.pdf}
\copyrightfilename{COLIEE2024camera/copyright-form-signed.pdf}
